Towards Zero-Shot Scale-Aware Monocular Depth Estimation

Monocular depth estimation is scale-ambiguous, and thus requires scale supervision to produce metric predictions. Even so, the resulting models will be geometry-specific, with learned scales that cannot be directly transferred across domains. Because of that, recent works focus instead on relative depth, eschewing scale in favor of improved up-to-scale zero-shot transfer. In this work we introduce ZeroDepth, a novel monocular depth estimation framework capable of predicting metric scale for arbitrary test images from different domains and camera parameters. This is achieved by (i) the use of input-level geometric embeddings that enable the network to learn a scale prior over objects; and (ii) decoupling the encoder and decoder stages, via a variational latent representation that is conditioned on single frame information. We evaluated ZeroDepth targeting both outdoor (KITTI, DDAD, nuScenes) and indoor (NYUv2) benchmarks, and achieved a new state-of-the-art in both settings using the same pre-trained model, outperforming methods that train on in-domain data and require test-time scaling to produce metric estimates.

==> figures/qualitative_indoor.tex <==

\begin{figure}[t!]
    \centering
    \subfloat{
    \includegraphics[width=0.24\textwidth]{assets/images/teaser/teaserkitti2.png}
    \includegraphics[width=0.24\textwidth]{assets/images/teaser/teaserkitti2.png}
    }
\caption{
\textbf{Indoor \Acronym depth estimation results.}
}
\end{figure}

==> tables/depth_all2.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%5

\captionsetup[table]{skip=6pt}

\begin{table*}[t!]
\small
\renewcommand{\arraystretch}{0.98}
\centering
{
\small
\setlength{\tabcolsep}{0.5em}
\begin{tabular}{l|ccc|c|cccc|ccc}
\toprule
\multirow{2}[2]{*}{\textbf{Method}} & 
\multicolumn{3}{c|}{\multirow{2}[2]{*}{\rotatebox{90}{\emph{\notsotiny{Supervision}}}}} & 
\multirow{2}[2]{*}{\rotatebox{90}{\emph{\notsotiny{Med. Scale}}}} & 
\multicolumn{4}{c|}{\textit{Lower is better}} &
\multicolumn{3}{c}{\textit{Higher is better}} 
\\
\cmidrule(lr){6-9} \cmidrule(lr){8-10}
& & & & &  
AbsRel &
SqRel &
RMSE &
RMSE$_{log}$ &
\scriptsize{$\delta < {1.25}$} &
\scriptsize{$\delta < {1.25}^2$} &
\scriptsize{$\delta < {1.25}^3$}\textbf{}
\\
\midrule
% \rowcolor{Gray}
\rowcolor{White}
Monodepth2~\cite{monodepth2}
& & M & & \cmark & 
0.115 & 0.903 & 4.863 & 0.193 & 0.877 & 0.959 & 0.981 
\\
\rowcolor{White}
& & M & & \cmark & 
0.111 & 0.785 & 4.601 & 0.189 & 0.878 & 0.960 & 0.982 
\\
\rowcolor{White}
\multirow{-2}{*}{PackNet-SfM~\cite{packnet}}
& & M+v & & \xmark & 
0.111 & 0.829 & 4.788 & 0.199 & 0.864 & 0.954 & 0.980 
\\
% \rowcolor{Gray}
\rowcolor{White}
GUDA~\cite{guda}
& & M+Sem & & \cmark & 
0.107 & 0.714 & 4.421 & --- & 0.883 & --- & --- 
\\
% \rowcolor{White}
% Wang \emph{et al.}~\cite{implicit_cues}
% & M & \cmark & 
% 0.106 & 0.799 & 4.662 & 0.187 & 0.889 & 0.961 & 0.982 
% \\
% \rowcolor{White}
% Johnston \emph{et al.}~\cite{johnston2020selfsupervised}
% & M & \cmark & 
% 0.106 & 0.861 & 4.699 & 0.185 & 0.889 & 0.962 & 0.982 
% \\
% \rowcolor{Gray}
\rowcolor{White}
MonoDEVSNet~\cite{virtualworld}
& & M & & \cmark & 
0.104 & 0.721 & 4.396 & 0.185 & 0.880 & 0.962 & 0.983 
\\
\rowcolor{White}
FeatDepth~\cite{shu2020featdepth}
& & M & & \cmark & 
0.104 & 0.729 & 4.481 & 0.179 & 0.893 & \sbestmed{0.965} & 0.982 
\\
% \rowcolor{Gray}
\rowcolor{White}
Guizilini \emph{et al.}~\cite{packnet-semguided}
& & M+Sem & & \cmark & 
\bestmed{0.102} & 0.698 & 4.381 & \sbestmed{0.178} & \sbestmed{0.896} & 0.964 & \sbestmed{0.984} 
\\
% \rowcolor{Gray}
\rowcolor{White}
& & & & \cmark & 
0.112 & 0.894 & 4.852 & 0.192 & 0.877 & 0.958 & 0.981 
\\
% \rowcolor{Gray}
\rowcolor{White}
\multirow{-2}{*}{Chawla \emph{et al.}~\cite{chawlavarma2021multimodal}}
& & \multirow{-2}{*}{M+GPS} & & \xmark & 
\sbestmet{0.109} & 0.860 & 4.855 & 0.198 & 0.865 & 0.954 & 0.980 
\\
\rowcolor{White}
& & & & \cmark & 
\sbestmed{0.103} & \sbestmed{0.654} & \sbestmed{4.300} & \sbestmed{0.178} & 0.891 & 0.966 & \sbestmed{0.984} 
\\
\rowcolor{White}
\multirow{-2}{*}{Swami \emph{et al.}~\cite{dowhatyoucan}}
& & \multirow{-2}{*}{M+V} & & \xmark & 
\sbestmet{0.109} & \sbestmet{0.702} & \sbestmet{4.409} & \sbestmet{0.185} & \sbestmet{0.876} & \sbestmet{0.962} & \sbestmet{0.984} 
\\
\midrule
& & & & \cmark & 
\bestmed{0.102} & \bestmed{\textbf{0.627}} & \bestmed{\textbf{4.044}} & \bestmed{\textbf{0.172}} & \bestmed{\textbf{0.910}} & \bestmed{\textbf{0.980}} & \bestmed{\textbf{0.996}}
\\
\multirow{-2}{*}{\textbf{\Acronym (outdoor)}}
& & \multirow{-2}{*}{---} & & \xmark & 
\bestmet{\textbf{0.100}} & \bestmet{\underline{0.662}} & \bestmet{\underline{4.213}} & \bestmet{\underline{0.181}} & \bestmet{\underline{0.899}} & \bestmet{\underline{0.973}} & \bestmet{\underline{0.992}}
\\
\bottomrule
\end{tabular}
}

\begin{tabular}{l|ccc|c|ccc|ccc}
\toprule
\multirow{2}[2]{*}{\textbf{Method}} & 
\multicolumn{3}{c|}{\multirow{2}[2]{*}{\rotatebox{90}{\emph{\notsotiny{Supervision}}}}} & 
\multirow{2}[2]{*}{\rotatebox{90}{\emph{\notsotiny{Med. Scale}}}} & 
\multicolumn{3}{c|}{\textit{DDAD}} &
\multicolumn{3}{c}{\textit{nuScenes}} 
\\
\cmidrule(lr){6-8} \cmidrule(lr){9-11}
& & & & &
AbsRel$\downarrow$ &
RMSE$\downarrow$ &
\scriptsize{$\delta < {1.25}$}$\uparrow$ &
AbsRel$\downarrow$ &
RMSE$\downarrow$ &
\scriptsize{$\delta < {1.25}$}$\uparrow$
\\
\midrule
% \rowcolor{Gray}
\rowcolor{White}
Monodepth2~\cite{monodepth2}
& & M & & \cmark &
% 0.217 & 3.641 & 12.962 & 0.323 & 0.699 & 0.877 & 0.939 
% 0.287 & 3.349 & 7.184 & 0.345 & 0.641 & 0.845 & 0.925 
0.217 & 12.962 & 0.699 & 
0.287 &  7.184 & 0.641
\\ 
\rowcolor{White}
PackNet-SfM~\cite{packnet}
& & M & & \cmark &
% 0.234 & 3.802 & 13.253 & 0.331 & 0.672 & 0.860 & 0.931 
% 0.309 & 2.891 & 7.994 & 0.390 & 0.547 & 0.796 & 0.899 
0.234 & 13.253 & 0.672 & 
0.309 & 7.994 & 0.547  
\\
% \rowcolor{Gray}
\rowcolor{White}
& & & & \cmark &
% 0.203 & 3.343 & 12.810 & 0.316 & 0.716 & 0.879 & 0.939
% 0.301 & 6.180 & 7.892 & 0.366 & 0.729 & 0.876 & 0.933 
0.203 & 12.810 & 0.716 & 
0.301 & 7.892 & 0.729
\\
% \rowcolor{Gray}
\rowcolor{White}
\multirow{-2}{*}{FSM~\cite{fsm}}
& & \multirow{-2}{*}{M+e} & & \xmark &
% 0.205 & 3.481 & 13.688 & 0.349 & 0.672 & 0.852 & 0.922 
% 0.319 & 7.534 & 7.860 & 0.362 & 0.716 & 0.874 & 0.931 
0.205 & 13.688 & 0.672 & 
0.319 &  7.860 & \sbestmet{0.716} 
\\
\rowcolor{White}
& & & & \cmark &
% 0.221 & 3.549 & 13.031 & 0.323 & 0.681 & 0.874 & 0.940 
% 0.271 & 4.496 & 7.391 & 0.346 & 0.726 & 0.879 & 0.934 
0.221 & 13.031 & 0.681 & 
0.271 &  7.391 & \sbestmed{0.726}
\\
\rowcolor{White}
\multirow{-2}{*}{VolumetricFusion~\cite{kim2022selfsupervised}}
& & \multirow{-2}{*}{M+e} & & \xmark &
% 0.218 & 3.660 & 13.327 & 0.339 & 0.674 & 0.862 & 0.932 
% 0.289 & 5.718 & 7.551 & 0.348 & 0.709 & 0.876 & 0.932 
0.218 & 13.327 & 0.674 & 
0.289 &  7.551 & 0.709
\\
% \rowcolor{Gray}
\rowcolor{White}
& & & & \cmark &
% 0.200 & 3.392 & 12.270 & 0.301 & 0.740 & 0.894 & 0.947 
% 0.245 & 3.067 & 6.835 & 0.321 & 0.719 & 0.878 & 0.935 
\sbestmed{0.200} & \sbestmed{12.270} & \sbestmed{0.740} & 
\sbestmed{0.245} &  \bestmed{\textbf{6.835}} & 0.719
\\
% \rowcolor{Gray}
\rowcolor{White}
\multirow{-2}{*}{SurroundDepth~\cite{wei2022surround}}
& & \multirow{-2}{*}{M+e} & & \xmark &
% 0.208 & 3.371 & 12.977 & 0.330 & 0.693 & 0.871 & 0.934 
% 0.280 & 4.401 & 7.467 & 0.364 & 0.661 & 0.844 & 0.917 
\sbestmet{0.208} & \sbestmet{12.977} & \sbestmet{0.693} & 
\sbestmet{0.280} &  \sbestmet{7.467} & 0.661
\\
\midrule
& & & & \cmark & 
% 0.160 & 2.610 & 10.814 & 0.258 & 0.811 & 0.924 & 0.961   
% 0.236 & 3.566 & 7.054 & 0.311 & 0.747 & 0.891 & 0.941
\bestmed{\textbf{0.160}} & \bestmed{\textbf{10.814}} & \bestmed{\underline{0.811}} & 
\bestmed{\textbf{0.236}} &  \sbestmed{\underline{7.054}} & \bestmed{\textbf{0.747}}  
\\
\multirow{-2}{*}{\textbf{\Acronym (outdoor)}}
& & \multirow{-2}{*}{---}&  & \xmark & 
% 0.161 & 2.633 & 11.034 & 0.272 & 0.813 & 0.915 & 0.956 
% 0.255 & 4.730 & 7.205 & 0.326 & 0.746 & 0.885 & 0.935  
\bestmet{\underline{0.161}} & \bestmet{\underline{11.034}} & \bestmet{\textbf{0.813}} & 
\bestmet{\underline{0.255}} &  \bestmet{7.205} & \bestmet{\underline{0.746}}
\\
\bottomrule
\end{tabular}
\caption{
\textbf{Depth estimation results on the KITTI~\cite{packnet} dataset.} \emph{Supervision} refers to the type of training supervision used in the target dataset (\emph{M} for monocular self-supervision, \emph{v} for velocity, \emph{V} for synthetic data with similar camera geometry, and \emph{Sem} for semantic segmentation), and \emph{Med. Scale} refers to the use of ground-truth median-scaling during evaluation. 
}
\label{tab:kitti}
\end{table*}

\captionsetup[table]{skip=6pt}

\begin{table*}[t!]
\small
\renewcommand{\arraystretch}{0.98}
\centering
{
\small
\setlength{\tabcolsep}{0.5em}
\begin{tabular}{l|ccc|c|ccc|ccc}
\toprule
\multirow{2}[2]{*}{\textbf{Method}} & 
\multicolumn{3}{c|}{\multirow{2}[2]{*}{\rotatebox{90}{\emph{\notsotiny{Supervision}}}}} & 
\multirow{2}[2]{*}{\rotatebox{90}{\emph{\notsotiny{Med. Scale}}}} & 
\multicolumn{3}{c|}{\textit{DDAD}} &
\multicolumn{3}{c}{\textit{nuScenes}} 
\\
\cmidrule(lr){6-8} \cmidrule(lr){9-11}
& & & & &
AbsRel$\downarrow$ &
RMSE$\downarrow$ &
\scriptsize{$\delta < {1.25}$}$\uparrow$ &
AbsRel$\downarrow$ &
RMSE$\downarrow$ &
\scriptsize{$\delta < {1.25}$}$\uparrow$
\\
\midrule
% \rowcolor{Gray}
\rowcolor{White}
Monodepth2~\cite{monodepth2}
& & M & & \cmark &
% 0.217 & 3.641 & 12.962 & 0.323 & 0.699 & 0.877 & 0.939 
% 0.287 & 3.349 & 7.184 & 0.345 & 0.641 & 0.845 & 0.925 
0.217 & 12.962 & 0.699 & 
0.287 &  7.184 & 0.641
\\ 
\rowcolor{White}
PackNet-SfM~\cite{packnet}
& & M & & \cmark &
% 0.234 & 3.802 & 13.253 & 0.331 & 0.672 & 0.860 & 0.931 
% 0.309 & 2.891 & 7.994 & 0.390 & 0.547 & 0.796 & 0.899 
0.234 & 13.253 & 0.672 & 
0.309 & 7.994 & 0.547  
\\
% \rowcolor{Gray}
\rowcolor{White}
& & & & \cmark &
% 0.203 & 3.343 & 12.810 & 0.316 & 0.716 & 0.879 & 0.939
% 0.301 & 6.180 & 7.892 & 0.366 & 0.729 & 0.876 & 0.933 
0.203 & 12.810 & 0.716 & 
0.301 & 7.892 & 0.729
\\
% \rowcolor{Gray}
\rowcolor{White}
\multirow{-2}{*}{FSM~\cite{fsm}}
& & \multirow{-2}{*}{M+e} & & \xmark &
% 0.205 & 3.481 & 13.688 & 0.349 & 0.672 & 0.852 & 0.922 
% 0.319 & 7.534 & 7.860 & 0.362 & 0.716 & 0.874 & 0.931 
0.205 & 13.688 & 0.672 & 
0.319 &  7.860 & \sbestmet{0.716} 
\\
\rowcolor{White}
& & & & \cmark &
% 0.221 & 3.549 & 13.031 & 0.323 & 0.681 & 0.874 & 0.940 
% 0.271 & 4.496 & 7.391 & 0.346 & 0.726 & 0.879 & 0.934 
0.221 & 13.031 & 0.681 & 
0.271 &  7.391 & \sbestmed{0.726}
\\
\rowcolor{White}
\multirow{-2}{*}{VolumetricFusion~\cite{kim2022selfsupervised}}
& & \multirow{-2}{*}{M+e} & & \xmark &
% 0.218 & 3.660 & 13.327 & 0.339 & 0.674 & 0.862 & 0.932 
% 0.289 & 5.718 & 7.551 & 0.348 & 0.709 & 0.876 & 0.932 
0.218 & 13.327 & 0.674 & 
0.289 &  7.551 & 0.709
\\
% \rowcolor{Gray}
\rowcolor{White}
& & & & \cmark &
% 0.200 & 3.392 & 12.270 & 0.301 & 0.740 & 0.894 & 0.947 
% 0.245 & 3.067 & 6.835 & 0.321 & 0.719 & 0.878 & 0.935 
\sbestmed{0.200} & \sbestmed{12.270} & \sbestmed{0.740} & 
\sbestmed{0.245} &  \bestmed{\textbf{6.835}} & 0.719
\\
% \rowcolor{Gray}
\rowcolor{White}
\multirow{-2}{*}{SurroundDepth~\cite{wei2022surround}}
& & \multirow{-2}{*}{M+e} & & \xmark &
% 0.208 & 3.371 & 12.977 & 0.330 & 0.693 & 0.871 & 0.934 
% 0.280 & 4.401 & 7.467 & 0.364 & 0.661 & 0.844 & 0.917 
\sbestmet{0.208} & \sbestmet{12.977} & \sbestmet{0.693} & 
\sbestmet{0.280} &  \sbestmet{7.467} & 0.661
\\
\midrule
& & & & \cmark & 
% 0.160 & 2.610 & 10.814 & 0.258 & 0.811 & 0.924 & 0.961   
% 0.236 & 3.566 & 7.054 & 0.311 & 0.747 & 0.891 & 0.941
\bestmed{\textbf{0.160}} & \bestmed{\textbf{10.814}} & \bestmed{\underline{0.811}} & 
\bestmed{\textbf{0.236}} &  \sbestmed{\underline{7.054}} & \bestmed{\textbf{0.747}}  
\\
\multirow{-2}{*}{\textbf{\Acronym (outdoor)}}
& & \multirow{-2}{*}{---}&  & \xmark & 
% 0.161 & 2.633 & 11.034 & 0.272 & 0.813 & 0.915 & 0.956 
% 0.255 & 4.730 & 7.205 & 0.326 & 0.746 & 0.885 & 0.935  
\bestmet{\underline{0.161}} & \bestmet{\underline{11.034}} & \bestmet{\textbf{0.813}} & 
\bestmet{\underline{0.255}} &  \bestmet{7.205} & \bestmet{\underline{0.746}}
\\
\bottomrule
\end{tabular}
}
\caption{
\textbf{Depth estimation results on the DDAD~\cite{packnet} and nuScenes~\cite{caesar2020nuscenes} datasets.} 
Reported results are the average of all $6$ cameras. \emph{Supervision} refers to the type of training supervision used in the target dataset (\emph{M} for monocular self-supervision, and \emph{e} for camera extrinsics), and \emph{Med. Scale} refers to the use of ground-truth median-scaling during evaluation. 
}
\label{tab:ddad_nuscenes}
\vspace{-5mm}
\end{table*}






==> tables/depth_ddad.tex <==

\captionsetup[table]{skip=6pt}

\begin{table*}[t!]
\small
\renewcommand{\arraystretch}{1.1}
\centering
{
\small
\setlength{\tabcolsep}{0.5em}
\begin{tabular}{l|c|c|cccc|ccc}
\toprule
\multirow{2}[2]{*}{\textbf{Method}} & 
\multirow{2}[2]{*}{\rotatebox{90}{\emph{\notsotiny{Supervision}}}} & 
\multirow{2}[2]{*}{\rotatebox{90}{\emph{\notsotiny{Med. Scale}}}} & 
\multicolumn{4}{c|}{\textit{Lower is better}} &
\multicolumn{3}{c}{\textit{Higher is better}} 
\\
\cmidrule(lr){4-7} \cmidrule(lr){8-10}
& & &
AbsRel &
SqRel &
RMSE &
RMSE$_{log}$ &
\scriptsize{$\delta < {1.25}$} &
\scriptsize{$\delta < {1.25}^2$} &
\scriptsize{$\delta < {1.25}^3$}
\\
\midrule
\rowcolor{Gray}
Monodepth2~\cite{monodepth2}
& M & \cmark &
0.217 & 3.641 & 12.962 & 0.323 & 0.699 & 0.877 & 0.939 
\\ 
\rowcolor{White}
PackNet-SfM~\cite{packnet}
& M & \cmark &
0.234 & 3.802 & 13.253 & 0.331 & 0.672 & 0.860 & 0.931 
\\
\rowcolor{Gray}
& & \cmark &
0.203 & 3.343 & 12.810 & 0.316 & 0.716 & 0.879 & 0.939
\\
\rowcolor{Gray}
\multirow{-2}{*}{FSM~\cite{fsm}}
& \multirow{-2}{*}{M+e} & \xmark &
0.205 & 3.481 & 13.688 & 0.349 & 0.672 & 0.852 & 0.922 
\\
\rowcolor{White}
& & \cmark &
0.221 & 3.549 & 13.031 & 0.323 & 0.681 & 0.874 & 0.940 
\\
\rowcolor{White}
\multirow{-2}{*}{VolumetricFusion~\cite{kim2022selfsupervised}}
& \multirow{-2}{*}{M+e} & \xmark &
0.218 & 3.660 & 13.327 & 0.339 & 0.674 & 0.862 & 0.932 
\\
\rowcolor{Gray}
& & \cmark &
0.200 & 3.392 & 12.270 & 0.301 & 0.740 & 0.894 & 0.947 
\\
\rowcolor{Gray}
\multirow{-2}{*}{SurroundDepth~\cite{wei2022surround}}
& \multirow{-2}{*}{M+e} & \xmark &
0.208 & 3.371 & 12.977 & 0.330 & 0.693 & 0.871 & 0.934 
\\
\midrule
& & \cmark & 
0.160 & 2.610 & 10.814 & 0.258 & 0.811 & 0.924 & 0.961   
\\
\multirow{-2}{*}{\textbf{Ours}}
& \multirow{-2}{*}{---} & \xmark & 
0.161 & 2.633 & 11.034 & 0.272 & 0.813 & 0.915 & 0.956 
\\
\bottomrule
\end{tabular}
}
\caption{
\textbf{Depth estimation results on the DDAD~\cite{packnet} dataset.} 
Reported results are the average of all $6$ cameras. \emph{Supervision} refers to the type of training supervision used in the target dataset (\emph{M} for monocular self-supervision, and \emph{e} for camera extrinsics), and \emph{Med. Scale} refers to the use of ground-truth median-scaling during evaluation. 
}
\label{tab:ddad}
\end{table*}

% \begin{table*}[t!]
% %\vspace{-4mm}
% \renewcommand{\arraystretch}{0.9}
% \centering
% {
% \small
% \setlength{\tabcolsep}{0.3em}
% \begin{tabular}{c|c|c|ccccc|ccc}
% \toprule
% & \multirow{2}{*}{\textbf{Input}} & \multirow{2}{*}{\textbf{Camera}} &
% \multicolumn{5}{|c|}{Lower is better $\downarrow$} &
% \multicolumn{3}{|c}{Higher is better $\uparrow$} \\
% & & & 
% Abs.Rel &
% Sqr.Rel &
% RMSE &
% RMSE$_{log}$ &
% SILog & 
% $\delta<1.25$ &
% $\delta<1.25^2$ &
% $\delta<1.25^3$\vspace{0.5mm}\\
% \toprule

% \parbox[t]{2mm}{\multirow{4}{*}{\rotatebox[origin=c]{90}{\textit{PackNet}}}} 
% & \multirow{4}{*}{RGB} 
% & 01 & 0.088 & 1.760 & 11.331 & 0.195 & 18.499 & 0.899 & 0.960 & 0.981 
% \\
% & & 05 & 0.130 & 2.025 & 10.472 & 0.268 & 25.273 & 0.832 & 0.927 & 0.960
% \\
% & & 06 & 0.151 & 2.485 & 10.680 & 0.307 & 28.007 & 0.791 & 0.904 & 0.944
% \\
% & & 09 & 0.132 & 2.362 & 12.497 & 0.261 & 24.551 & 0.821 & 0.925 & 0.962
% \\
% \midrule
% \midrule
% \parbox[t]{2mm}{\multirow{9}{*}{\rotatebox[origin=c]{90}{\textit{PackNet-SAN}}}} 
% & \multirow{5}{*}{RGB} 
% & 01 & 0.083 & 1.575 & 10.693 & 0.185 & 17.767 & 0.911 & 0.967 & 0.987 
% \\
% & & 05 & 0.127 & 1.863 & 10.210 & 0.263 & 24.966 & 0.841 & 0.931 & 0.973
% \\
% & & 06 & 0.145 & 2.307 & 10.493 & 0.298 & 27.491 & 0.804 & 0.911 & 0.968
% \\
% & & 09 & 0.119 & 1.979 & 12.010 & 0.256 & 24.295 & 0.844 & 0.936 & 0.978
% \\
% \cmidrule{3-11}
% & & {\textit{Avg. Improv.}} & \textit{5.45\%} & \textit{10.47\%} & \textit{3.44\%} & \textit{2.96\%} & \textit{2.01\%} & \textit{1.71\%} & \textit{0.78\%} & \textit{1.54\%}
% \\
% \cmidrule{2-11}
% \cmidrule{2-11}
% & \multirow{4}{*}{RGB+D} 
% & 01 & 0.052 & 0.933 & 8.683 & 0.153 & 14.920 & 0.955 & 0.978 & 0.987 
% \\
% & & 05 & 0.072 & 1.097 & 7.950 & 0.207 & 20.375 & 0.928 & 0.958 & 0.973
% \\
% & & 06 & 0.081 & 1.255 & 7.994 & 0.232 & 22.675 & 0.922 & 0.955 & 0.969
% \\
% & & 09 & 0.067 & 1.131 & 9.052 & 0.189 & 18.481 & 0.934 & 0.966 & 0.979
% \\

% % \midrule
% % \midrule

% % \parbox[t]{2mm}{\multirow{6}{*}{\rotatebox[origin=c]{90}{\textit{Official}}}}

% % % & Gansbeke et al. \cite{wvangansbeke_depth_2019} & RGB
% % % & --- & --- & 3.233 & --- & --- & --- & --- & ---

% % % \\\cmidrule{2-11}

% % % & Ferstl et al. \cite{completionnonlearning} & RGB+D
% % % & --- & --- & 2.761 & --- & --- & --- & --- & --- 
% % % \\
% % % & Zhang et al. \cite{zhang2018deepdepth} & RGB+D
% % % & --- & --- & 1.312 & --- & --- & --- & --- & --- 
% % % \\
% % % & Huang et al. \cite{hmsnet} & RGB+D
% % % & --- & --- & 0.883 & --- & --- & --- & --- & --- 
% % % \\
% % % & Eldesokey et al. \cite{propconf} & RGB+D
% % % & --- & --- & 0.908 & --- & --- & --- & --- & --- 
% % % \\

% % & Gansbeke et al. \cite{wvangansbeke_depth_2019} & RGB+D
% % & \textbf{0.011} & \textbf{0.024} & \textbf{0.802} & \textbf{0.029} & \textbf{2.849} & \textbf{0.998} & \textbf{0.999} & \textbf{1.000} 

% % \\\cmidrule{2-11}

% % & \multirow{2}{*}{BTS-SAN \cite{lee2019big}} & RGB
% % & 0.061 & 0.247 & 2.797 & 0.096 & 9.323 & 0.957 & 0.993 & 0.998 
% % \\
% % & & RGB+D
% % & 0.020 & 0.035 & 1.061 & 0.037 & 3.685 & 0.996 & \textbf{0.999} & \textbf{1.000} 

% % \\\cmidrule{2-11}

% % & \multirow{2}{*}{PackNet-SAN \cite{packnet}} & RGB
% % & \textbf{0.055} & \textbf{0.223} & \textbf{2.611} & \textbf{0.093} & \textbf{8.689} & \textbf{0.962} & \textbf{0.993} & \textbf{0.998}

% % \\

% % & & RGB+D
% % & \underline{0.014} & \underline{0.026} & \underline{0.889} & \underline{0.031} & \underline{3.109} & \underline{0.997} & \textbf{0.999} & \textbf{1.000}
% % \\

% %\parbox[t]{2mm}{\multirow{11}{*}{\rotatebox[origin=c]{90}{Improved~\cite{gtkitti}}}}

% \bottomrule

% \end{tabular}
% }
% \caption{\textbf{Depth estimation results on DDAD} using PackNet-SAN, with the same model trained on four cameras considering distances up to 200m. For the RGB+D experiments, a sparsity level of 20\% was used for input depth maps.} 
% \label{tab:depth_ddad}
% \end{table*}




==> tables/depth_ddad_nuscenes.tex <==

\captionsetup[table]{skip=6pt}

\begin{table*}[t!]
\small
\renewcommand{\arraystretch}{0.98}
\centering
{
\small
\setlength{\tabcolsep}{0.5em}
\begin{tabular}{l|c|c|ccc|ccc}
\toprule
\multirow{2}[2]{*}{\textbf{Method}} & 
\multirow{2}[2]{*}{\rotatebox{90}{\emph{\notsotiny{Supervision}}}} & 
\multirow{2}[2]{*}{\rotatebox{90}{\emph{\notsotiny{Med. Scale}}}} & 
\multicolumn{3}{c|}{\textit{DDAD}} &
\multicolumn{3}{c}{\textit{nuScenes}} 
\\
\cmidrule(lr){4-6} \cmidrule(lr){7-9}
& & &
AbsRel$\downarrow$ &
RMSE$\downarrow$ &
\scriptsize{$\delta < {1.25}$}$\uparrow$ &
AbsRel$\downarrow$ &
RMSE$\downarrow$ &
\scriptsize{$\delta < {1.25}$}$\uparrow$
\\
\midrule
% \rowcolor{Gray}
\rowcolor{White}
Monodepth2~\cite{monodepth2}
& M & \cmark &
% 0.217 & 3.641 & 12.962 & 0.323 & 0.699 & 0.877 & 0.939 
% 0.287 & 3.349 & 7.184 & 0.345 & 0.641 & 0.845 & 0.925 
0.217 & 12.962 & 0.699 & 
0.287 &  7.184 & 0.641
\\ 
\rowcolor{White}
PackNet-SfM~\cite{packnet}
& M & \cmark &
% 0.234 & 3.802 & 13.253 & 0.331 & 0.672 & 0.860 & 0.931 
% 0.309 & 2.891 & 7.994 & 0.390 & 0.547 & 0.796 & 0.899 
0.234 & 13.253 & 0.672 & 
0.309 & 7.994 & 0.547  
\\
% \rowcolor{Gray}
\rowcolor{White}
& & \cmark &
% 0.203 & 3.343 & 12.810 & 0.316 & 0.716 & 0.879 & 0.939
% 0.301 & 6.180 & 7.892 & 0.366 & 0.729 & 0.876 & 0.933 
0.203 & 12.810 & 0.716 & 
0.301 & 7.892 & 0.729
\\
% \rowcolor{Gray}
\rowcolor{White}
\multirow{-2}{*}{FSM~\cite{fsm}}
& \multirow{-2}{*}{M+e} & \xmark &
% 0.205 & 3.481 & 13.688 & 0.349 & 0.672 & 0.852 & 0.922 
% 0.319 & 7.534 & 7.860 & 0.362 & 0.716 & 0.874 & 0.931 
0.205 & 13.688 & 0.672 & 
0.319 &  7.860 & \sbestmet{0.716} 
\\
\rowcolor{White}
& & \cmark &
% 0.221 & 3.549 & 13.031 & 0.323 & 0.681 & 0.874 & 0.940 
% 0.271 & 4.496 & 7.391 & 0.346 & 0.726 & 0.879 & 0.934 
0.221 & 13.031 & 0.681 & 
0.271 &  7.391 & \sbestmed{0.726}
\\
\rowcolor{White}
\multirow{-2}{*}{VolumetricFusion~\cite{kim2022selfsupervised}}
& \multirow{-2}{*}{M+e} & \xmark &
% 0.218 & 3.660 & 13.327 & 0.339 & 0.674 & 0.862 & 0.932 
% 0.289 & 5.718 & 7.551 & 0.348 & 0.709 & 0.876 & 0.932 
0.218 & 13.327 & 0.674 & 
0.289 &  7.551 & 0.709
\\
% \rowcolor{Gray}
\rowcolor{White}
& & \cmark &
% 0.200 & 3.392 & 12.270 & 0.301 & 0.740 & 0.894 & 0.947 
% 0.245 & 3.067 & 6.835 & 0.321 & 0.719 & 0.878 & 0.935 
\sbestmed{0.200} & \sbestmed{12.270} & \sbestmed{0.740} & 
\sbestmed{0.245} &  \bestmed{\textbf{6.835}} & 0.719
\\
% \rowcolor{Gray}
\rowcolor{White}
\multirow{-2}{*}{SurroundDepth~\cite{wei2022surround}}
& \multirow{-2}{*}{M+e} & \xmark &
% 0.208 & 3.371 & 12.977 & 0.330 & 0.693 & 0.871 & 0.934 
% 0.280 & 4.401 & 7.467 & 0.364 & 0.661 & 0.844 & 0.917 
\sbestmet{0.208} & \sbestmet{12.977} & \sbestmet{0.693} & 
\sbestmet{0.280} &  \sbestmet{7.467} & 0.661
\\
\midrule
& & \cmark & 
% 0.160 & 2.610 & 10.814 & 0.258 & 0.811 & 0.924 & 0.961   
% 0.236 & 3.566 & 7.054 & 0.311 & 0.747 & 0.891 & 0.941
\bestmed{\textbf{0.160}} & \bestmed{\textbf{10.814}} & \bestmed{\underline{0.811}} & 
\bestmed{\textbf{0.236}} &  \sbestmed{\underline{7.054}} & \bestmed{\textbf{0.747}}  
\\
\multirow{-2}{*}{\textbf{\Acronym (outdoor)}}
& \multirow{-2}{*}{---} & \xmark & 
% 0.161 & 2.633 & 11.034 & 0.272 & 0.813 & 0.915 & 0.956 
% 0.255 & 4.730 & 7.205 & 0.326 & 0.746 & 0.885 & 0.935  
\bestmet{\underline{0.161}} & \bestmet{\underline{11.034}} & \bestmet{\textbf{0.813}} & 
\bestmet{\underline{0.255}} &  \bestmet{7.205} & \bestmet{\underline{0.746}}
\\
\bottomrule
\end{tabular}
}
\caption{
\textbf{Depth estimation results on the DDAD~\cite{packnet} and nuScenes~\cite{caesar2020nuscenes} datasets.} 
Reported results are the average of all $6$ cameras. \emph{Supervision} refers to the type of training supervision used in the target dataset (\emph{M} for monocular self-supervision, and \emph{e} for camera extrinsics), and \emph{Med. Scale} refers to the use of ground-truth median-scaling during evaluation. 
}
\label{tab:ddad_nuscenes}
\vspace{-5mm}
\end{table*}





==> tables/depth_kitti.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%5

\captionsetup[table]{skip=6pt}

\begin{table*}[t!]
\small
\renewcommand{\arraystretch}{0.98}
\centering
{
\small
\setlength{\tabcolsep}{0.5em}
\begin{tabular}{l|c|c|cccc|ccc}
\toprule
\multirow{2}[2]{*}{\textbf{Method}} & 
\multirow{2}[2]{*}{\rotatebox{90}{\emph{\notsotiny{Supervision}}}} & 
\multirow{2}[2]{*}{\rotatebox{90}{\emph{\notsotiny{Med. Scale}}}} & 
\multicolumn{4}{c|}{\textit{Lower is better}} &
\multicolumn{3}{c}{\textit{Higher is better}} 
\\
\cmidrule(lr){4-7} \cmidrule(lr){8-10}
& & &  
AbsRel &
SqRel &
RMSE &
RMSE$_{log}$ &
\scriptsize{$\delta < {1.25}$} &
\scriptsize{$\delta < {1.25}^2$} &
\scriptsize{$\delta < {1.25}^3$}\textbf{}
\\
\midrule
% \rowcolor{Gray}
\rowcolor{White}
Monodepth2~\cite{monodepth2}
& M & \cmark & 
0.115 & 0.903 & 4.863 & 0.193 & 0.877 & 0.959 & 0.981 
\\
\rowcolor{White}
& M & \cmark & 
0.111 & 0.785 & 4.601 & 0.189 & 0.878 & 0.960 & 0.982 
\\
\rowcolor{White}
\multirow{-2}{*}{PackNet-SfM~\cite{packnet}}
& M+v & \xmark & 
0.111 & 0.829 & 4.788 & 0.199 & 0.864 & 0.954 & 0.980 
\\
% \rowcolor{Gray}
\rowcolor{White}
GUDA~\cite{guda}
& M+Sem & \cmark & 
0.107 & 0.714 & 4.421 & --- & 0.883 & --- & --- 
\\
% \rowcolor{White}
% Wang \emph{et al.}~\cite{implicit_cues}
% & M & \cmark & 
% 0.106 & 0.799 & 4.662 & 0.187 & 0.889 & 0.961 & 0.982 
% \\
% \rowcolor{White}
% Johnston \emph{et al.}~\cite{johnston2020selfsupervised}
% & M & \cmark & 
% 0.106 & 0.861 & 4.699 & 0.185 & 0.889 & 0.962 & 0.982 
% \\
% \rowcolor{Gray}
\rowcolor{White}
MonoDEVSNet~\cite{virtualworld}
& M & \cmark & 
0.104 & 0.721 & 4.396 & 0.185 & 0.880 & 0.962 & 0.983 
\\
\rowcolor{White}
FeatDepth~\cite{shu2020featdepth}
& M & \cmark & 
0.104 & 0.729 & 4.481 & 0.179 & 0.893 & \sbestmed{0.965} & 0.982 
\\
% \rowcolor{Gray}
\rowcolor{White}
Guizilini \emph{et al.}~\cite{packnet-semguided}
& M+Sem & \cmark & 
\bestmed{0.102} & 0.698 & 4.381 & \sbestmed{0.178} & \sbestmed{0.896} & 0.964 & \sbestmed{0.984} 
\\
% \rowcolor{Gray}
\rowcolor{White}
& & \cmark & 
0.112 & 0.894 & 4.852 & 0.192 & 0.877 & 0.958 & 0.981 
\\
% \rowcolor{Gray}
\rowcolor{White}
\multirow{-2}{*}{Chawla \emph{et al.}~\cite{chawlavarma2021multimodal}}
& \multirow{-2}{*}{M+GPS} & \xmark & 
\sbestmet{0.109} & 0.860 & 4.855 & 0.198 & 0.865 & 0.954 & 0.980 
\\
\rowcolor{White}
& & \cmark & 
\sbestmed{0.103} & \sbestmed{0.654} & \sbestmed{4.300} & \sbestmed{0.178} & 0.891 & 0.966 & \sbestmed{0.984} 
\\
\rowcolor{White}
\multirow{-2}{*}{Swami \emph{et al.}~\cite{dowhatyoucan}}
& \multirow{-2}{*}{M+V} & \xmark & 
\sbestmet{0.109} & \sbestmet{0.702} & \sbestmet{4.409} & \sbestmet{0.185} & \sbestmet{0.876} & \sbestmet{0.962} & \sbestmet{0.984} 
\\
\midrule
& & \cmark & 
\bestmed{0.102} & \bestmed{\textbf{0.627}} & \bestmed{\textbf{4.044}} & \bestmed{\textbf{0.172}} & \bestmed{\textbf{0.910}} & \bestmed{\textbf{0.980}} & \bestmed{\textbf{0.996}}
\\
\multirow{-2}{*}{\textbf{\Acronym (outdoor)}}
& \multirow{-2}{*}{---} & \xmark & 
\bestmet{\textbf{0.100}} & \bestmet{\underline{0.662}} & \bestmet{\underline{4.213}} & \bestmet{\underline{0.181}} & \bestmet{\underline{0.899}} & \bestmet{\underline{0.973}} & \bestmet{\underline{0.992}}
\\
\bottomrule
\end{tabular}
}
\caption{
\textbf{Depth estimation results on the KITTI~\cite{packnet} dataset.} \emph{Supervision} refers to the type of training supervision used in the target dataset (\emph{M} for monocular self-supervision, \emph{v} for velocity, \emph{V} for synthetic data with similar camera geometry, and \emph{Sem} for semantic segmentation), and \emph{Med. Scale} refers to the use of ground-truth median-scaling during evaluation. 
}
\label{tab:kitti}
\end{table*}



% \captionsetup[table]{skip=6pt}

% \begin{table*}[t!]
% \small
% \renewcommand{\arraystretch}{0.9}
% \centering
% {
% \small
% \setlength{\tabcolsep}{0.3em}
% \begin{tabular}{l|c|c|c|cccc|ccc}
% \toprule
% \multirow{2}[2]{*}{\textbf{Method}} & 
% \multirow{2}[2]{*}{\rotatebox{90}{\scriptsize{Multi-Fr.}}} & 
% \multirow{2}[2]{*}{\rotatebox{90}{\scriptsize{Synthetic}}} & 
% \multirow{2}[2]{*}{\rotatebox{90}{\scriptsize{Semantic}}} & 
% \multicolumn{4}{c|}{\textit{Lower is better}} &
% \multicolumn{3}{c}{\textit{Higher is better}} 
% \\
% \cmidrule(lr){5-8} \cmidrule(lr){9-11}
% & & & &
% AbsRel &
% SqRel &
% RMSE &
% RMSE$_{log}$ &
% $\delta < {1.25}$ &
% $\delta < {1.25}^2$ &
% $\delta < {1.25}^3$
% \\
% \midrule
% % Ranjan \emph{et al.} \cite{competi_colab}
% % & & & 
% % & 0.148 & 1.149 & 5.464 & 0.226 & 0.815 & 0.935 & 0.973 
% % \\
% % EPC++ \cite{epc++}
% % & & & 
% % & 0.141 & 1.029 & 5.350 & 0.216 & 0.816 & 0.941 & 0.976 
% % \\
% Struct2Depth \cite{casser2018depth}
% & & & \checkmark
% & 0.141 & 1.026 & 5.291 & 0.215 & 0.816 & 0.945 & 0.979 
% \\
% % Li \emph{et al.} \cite{dynamic_scenes}
% % & & & 
% % & 0.130 & 0.950 & 5.138 & 0.209 & 0.843 & 0.948 & 0.978 
% % \\
% Gordon \emph{et al.} \cite{gordon2019depth}
% & & & \checkmark
% & 0.128 & 0.959 & 5.230 & 0.212 & 0.845 & 0.947 & 0.976 
% \\
% GASDA \cite{gasda}
% & & \checkmark &
% & 0.120 & 1.022 & 5.162 & 0.215 & 0.848 & 0.944 & 0.974
% \\
% SharinGAN \cite{sharingan}
% & & \checkmark &
% & 0.116 & 0.939 & 5.068 & 0.203 & 0.850 & 0.948 & 0.978
% \\
% Monodepth2 \cite{monodepth2}
% & & & 
% & 0.115 & 0.903 & 4.863 & 0.193 & 0.877 & 0.959 & 0.981 
% \\
% Patil \emph{et al.} \cite{forget_past}
% & \checkmark & & 
% & 0.111 & 0.821 & 4.650 & 0.187 & 0.883 & 0.961 & 0.982 
% \\
% PackNet-SFM \cite{packnet}
% & & & 
% & 0.111 & 0.785 & 4.601 & 0.189 & 0.878 & 0.960 & 0.982 
% \\
% GUDA \cite{guda}
% & & \checkmark & 
% & 0.107 & 0.714 & 4.421 & --- & 0.883 & --- & --- 
% \\
% Johnston \emph{et al.} \cite{johnston2020selfsupervised}
% & & & 
% & 0.106 & 0.861 & 4.699 & 0.185 & 0.889 & 0.962 & 0.982 
% \\
% Wang \emph{et al.} \cite{implicit_cues}
% & \checkmark & & 
% & 0.106 & 0.799 & 4.662 & 0.187 & 0.889 & 0.961 & 0.982 
% \\
% MonoDEVSNet \cite{virtualworld}
% & & \checkmark &
% & 0.104 & 0.721 & 4.396 & 0.185 & 0.880 & 0.962 & \underline{0.983}
% \\
% TC-Depth \cite{ruhkamp2021attention}
% & \checkmark & &
% & 0.103 & 0.746 & 4.483 & 0.185 & 0.894 & --- & \underline{0.983}
% \\
% Guizilini \emph{et al.} \cite{packnet-semguided}
% & & & \checkmark
% & 0.102 & \underline{0.698} & \underline{4.381} & 0.178 & 0.896 & 0.964 & \textbf{0.984} 
% \\
% ManyDepth \cite{manydepth} 
% & \checkmark & & 
% & \underline{0.098} & 0.770 & 4.459 & \underline{0.176} & \underline{0.900} & \underline{0.965} & \underline{0.983} 
% \\
% \midrule
% \textbf{DepthFormer} 
% & \checkmark & & 
% % & \textbf{0.094} & \underline{0.712} & \textbf{4.243} & \underline{0.177} & \textbf{0.900} & \textbf{0.966} & \textbf{0.985} 
% & \textbf{0.090} & \textbf{0.661} & \textbf{4.149} & \textbf{0.175} & \textbf{0.905} & \textbf{0.967} & \textbf{0.984} 
% \\
% \bottomrule
% \end{tabular}
% }
% \caption{
% \textbf{Depth estimation results} on the KITTI \emph{Eigen} test split \cite{eigen2014depth}, for distances up to 80m with the \emph{Garg} crop~\cite{garg2016unsupervised} and half resolution ($640 \times 192$ or similar). \emph{Multi-Fr.} indicates the use of multiple frames at test time; \emph{Synthetic} the use of additional synthetic training data; and \emph{Semantic} the use of additional semantic information. 
% }
% \label{table:kitti_depth_selfsup}
% \vspace{-4mm}
% \end{table*}


==> tables/depth_nuscenes.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%5

\captionsetup[table]{skip=6pt}

\begin{table*}[t!]
\small
\renewcommand{\arraystretch}{1.1}
\centering
{
\small
\setlength{\tabcolsep}{0.3em}
\begin{tabular}{l|c|c|cccc|ccc}
\toprule
\multirow{2}[2]{*}{\textbf{Method}} & 
\multirow{2}[2]{*}{\rotatebox{90}{\emph{\notsotiny{Supervision}}}} & 
\multirow{2}[2]{*}{\rotatebox{90}{\emph{\notsotiny{Med. Scale}}}} & 
\multicolumn{4}{c|}{\textit{Lower is better}} &
\multicolumn{3}{c}{\textit{Higher is better}} 
\\
\cmidrule(lr){4-7} \cmidrule(lr){8-10}
& & & 
AbsRel &
SqRel &
RMSE &
RMSE$_{log}$ &
\scriptsize{$\delta < {1.25}$} &
\scriptsize{$\delta < {1.25}^2$} &
\scriptsize{$\delta < {1.25}^3$}
\\
\midrule
\rowcolor{Gray}
Monodepth2~\cite{monodepth2}
& M & \cmark & 
0.287 & 3.349 & 7.184 & 0.345 & 0.641 & 0.845 & 0.925 
\\
\rowcolor{White}
PackNet-SfM~\cite{packnet}
& M & \cmark &
0.309 & 2.891 & 7.994 & 0.390 & 0.547 & 0.796 & 0.899 
\\
\rowcolor{Gray}
& & \cmark &
0.301 & 6.180 & 7.892 & 0.366 & 0.729 & 0.876 & 0.933 
% 0.312 & 8.697 & 9.288 & 0.371 & 0.686 & 9.850 & 0.917 
\\
\rowcolor{Gray}
\multirow{-2}{*}{FSM~\cite{fsm}}
& \multirow{-2}{*}{M+e} & \xmark & 
0.319 & 7.534 & 7.860 & 0.362 & 0.716 & 0.874 & 0.931 
% 0.323 & 9.816 & 9.176 & 0.405 & 0.619 & 0.800 & 0.876 
\\
\rowcolor{White}
& & \cmark & 
0.271 & 4.496 & 7.391 & 0.346 & 0.726 & 0.879 & 0.934 
\\
\rowcolor{White}
\multirow{-2}{*}{VolumetricFusion~\cite{kim2022selfsupervised}}
& \multirow{-2}{*}{M+e} & \xmark & 
0.289 & 5.718 & 7.551 & 0.348 & 0.709 & 0.876 & 0.932 
\\
\rowcolor{Gray}
& & \cmark & 
0.245 & 3.067 & 6.835 & 0.321 & 0.719 & 0.878 & 0.935 
\\
\rowcolor{Gray}
\multirow{-2}{*}{SurroundDepth~\cite{wei2022surround}}
& \multirow{-2}{*}{M+e} & \xmark & 
0.280 & 4.401 & 7.467 & 0.364 & 0.661 & 0.844 & 0.917 
\\
\midrule
& & \cmark & 
0.236 & 3.566 & 7.054 & 0.311 & 0.747 & 0.891 & 0.941
\\
\multirow{-2}{*}{\textbf{Ours}}
& \multirow{-2}{*}{---} & \xmark & 
0.255 & 4.730 & 7.205 & 0.326 & 0.746 & 0.885 & 0.935  
\\
\bottomrule
\end{tabular}
}
\caption{
\textbf{Depth estimation results on the nuScenes~\cite{caesar2020nuscenes} dataset.}
Reported results are the average of all $6$ cameras. \emph{Supervision} refers to the type of training supervision used in the target dataset (\emph{M} for monocular self-supervision, and \emph{e} for camera extrinsics), and \emph{Med. Scale} refers to the use of ground-truth median-scaling during evaluation. 
}
\label{tab:nuscenes}
\end{table*}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%5

% \begin{table*}[t!]
% %\vspace{-4mm}
% \renewcommand{\arraystretch}{0.9}
% \centering
% {
% \small
% \setlength{\tabcolsep}{0.3em}
% \begin{tabular}{c|c|c|ccccc|ccc}
% \toprule
% & \multirow{2}{*}{\textbf{Input}} & \multirow{2}{*}{\textbf{Camera}} &
% \multicolumn{5}{|c|}{Lower is better $\downarrow$} &
% \multicolumn{3}{|c}{Higher is better $\uparrow$} \\
% & & & 
% Abs.Rel &
% Sqr.Rel &
% RMSE &
% RMSE$_{log}$ &
% SILog & 
% $\delta<1.25$ &
% $\delta<1.25^2$ &
% $\delta<1.25^3$\vspace{0.5mm}\\
% \toprule

% \parbox[t]{2mm}{\multirow{4}{*}{\rotatebox[origin=c]{90}{\textit{PackNet}}}} 
% & \multirow{4}{*}{RGB} 
% & 01 & 0.088 & 1.760 & 11.331 & 0.195 & 18.499 & 0.899 & 0.960 & 0.981 
% \\
% & & 05 & 0.130 & 2.025 & 10.472 & 0.268 & 25.273 & 0.832 & 0.927 & 0.960
% \\
% & & 06 & 0.151 & 2.485 & 10.680 & 0.307 & 28.007 & 0.791 & 0.904 & 0.944
% \\
% & & 09 & 0.132 & 2.362 & 12.497 & 0.261 & 24.551 & 0.821 & 0.925 & 0.962
% \\
% \midrule
% \midrule
% \parbox[t]{2mm}{\multirow{9}{*}{\rotatebox[origin=c]{90}{\textit{PackNet-SAN}}}} 
% & \multirow{5}{*}{RGB} 
% & 01 & 0.083 & 1.575 & 10.693 & 0.185 & 17.767 & 0.911 & 0.967 & 0.987 
% \\
% & & 05 & 0.127 & 1.863 & 10.210 & 0.263 & 24.966 & 0.841 & 0.931 & 0.973
% \\
% & & 06 & 0.145 & 2.307 & 10.493 & 0.298 & 27.491 & 0.804 & 0.911 & 0.968
% \\
% & & 09 & 0.119 & 1.979 & 12.010 & 0.256 & 24.295 & 0.844 & 0.936 & 0.978
% \\
% \cmidrule{3-11}
% & & {\textit{Avg. Improv.}} & \textit{5.45\%} & \textit{10.47\%} & \textit{3.44\%} & \textit{2.96\%} & \textit{2.01\%} & \textit{1.71\%} & \textit{0.78\%} & \textit{1.54\%}
% \\
% \cmidrule{2-11}
% \cmidrule{2-11}
% & \multirow{4}{*}{RGB+D} 
% & 01 & 0.052 & 0.933 & 8.683 & 0.153 & 14.920 & 0.955 & 0.978 & 0.987 
% \\
% & & 05 & 0.072 & 1.097 & 7.950 & 0.207 & 20.375 & 0.928 & 0.958 & 0.973
% \\
% & & 06 & 0.081 & 1.255 & 7.994 & 0.232 & 22.675 & 0.922 & 0.955 & 0.969
% \\
% & & 09 & 0.067 & 1.131 & 9.052 & 0.189 & 18.481 & 0.934 & 0.966 & 0.979
% \\

% % \midrule
% % \midrule

% % \parbox[t]{2mm}{\multirow{6}{*}{\rotatebox[origin=c]{90}{\textit{Official}}}}

% % % & Gansbeke et al. \cite{wvangansbeke_depth_2019} & RGB
% % % & --- & --- & 3.233 & --- & --- & --- & --- & ---

% % % \\\cmidrule{2-11}

% % % & Ferstl et al. \cite{completionnonlearning} & RGB+D
% % % & --- & --- & 2.761 & --- & --- & --- & --- & --- 
% % % \\
% % % & Zhang et al. \cite{zhang2018deepdepth} & RGB+D
% % % & --- & --- & 1.312 & --- & --- & --- & --- & --- 
% % % \\
% % % & Huang et al. \cite{hmsnet} & RGB+D
% % % & --- & --- & 0.883 & --- & --- & --- & --- & --- 
% % % \\
% % % & Eldesokey et al. \cite{propconf} & RGB+D
% % % & --- & --- & 0.908 & --- & --- & --- & --- & --- 
% % % \\

% % & Gansbeke et al. \cite{wvangansbeke_depth_2019} & RGB+D
% % & \textbf{0.011} & \textbf{0.024} & \textbf{0.802} & \textbf{0.029} & \textbf{2.849} & \textbf{0.998} & \textbf{0.999} & \textbf{1.000} 

% % \\\cmidrule{2-11}

% % & \multirow{2}{*}{BTS-SAN \cite{lee2019big}} & RGB
% % & 0.061 & 0.247 & 2.797 & 0.096 & 9.323 & 0.957 & 0.993 & 0.998 
% % \\
% % & & RGB+D
% % & 0.020 & 0.035 & 1.061 & 0.037 & 3.685 & 0.996 & \textbf{0.999} & \textbf{1.000} 

% % \\\cmidrule{2-11}

% % & \multirow{2}{*}{PackNet-SAN \cite{packnet}} & RGB
% % & \textbf{0.055} & \textbf{0.223} & \textbf{2.611} & \textbf{0.093} & \textbf{8.689} & \textbf{0.962} & \textbf{0.993} & \textbf{0.998}

% % \\

% % & & RGB+D
% % & \underline{0.014} & \underline{0.026} & \underline{0.889} & \underline{0.031} & \underline{3.109} & \underline{0.997} & \textbf{0.999} & \textbf{1.000}
% % \\

% %\parbox[t]{2mm}{\multirow{11}{*}{\rotatebox[origin=c]{90}{Improved~\cite{gtkitti}}}}

% \bottomrule

% \end{tabular}
% }
% \caption{\textbf{Depth estimation results on DDAD} using PackNet-SAN, with the same model trained on four cameras considering distances up to 200m. For the RGB+D experiments, a sparsity level of 20\% was used for input depth maps.} 
% \label{tab:depth_nuscenes}
% \end{table*}




==> tables/depth_waymo.tex <==

\captionsetup[table]{skip=6pt}

\begin{table*}[t!]
\small
\renewcommand{\arraystretch}{1.1}
\centering
{
\small
\setlength{\tabcolsep}{0.3em}
\begin{tabular}{l|c|c|cccc|ccc}
\toprule
\multirow{2}[2]{*}{\textbf{Method}} & 
\multirow{2}[2]{*}{\rotatebox{90}{\emph{\notsotiny{Supervision}}}} & 
\multirow{2}[2]{*}{\rotatebox{90}{\emph{\notsotiny{Med. Scale}}}} & 
\multicolumn{4}{c|}{\textit{Lower is better}} &
\multicolumn{3}{c}{\textit{Higher is better}} 
\\
\cmidrule(lr){4-7} \cmidrule(lr){8-10}
& & & 
AbsRel &
SqRel &
RMSE &
RMSE$_{log}$ &
\scriptsize{$\delta < {1.25}$} &
\scriptsize{$\delta < {1.25}^2$} &
\scriptsize{$\delta < {1.25}^3$}
\\
\midrule
% \rowcolor{Gray}
% Monodepth2~\cite{monodepth2}
% & & \cmark & 
% & & & & & & 
% \\
% \rowcolor{White}
% PackNet-SfM~\cite{packnet}
% & & \cmark &
% & & & & & & 
% \\
% \midrule
& & \cmark & 
0.196 & 2.946 & 7.314 & 0.264 & 0.752 & 0.910 & 0.957 
\\
\multirow{-2}{*}{\textbf{Ours}}
& & \xmark & 
0.239 & 3.756 & 8.043 & 0.294 & 0.713 & 0.889 & 0.943  
\\
\bottomrule
\end{tabular}
}
\caption{
\textbf{Depth estimation results on the Waymo~\cite{waymo} dataset.}
}
\label{tab:waymo}
\end{table*}


==> tables/fine-tuning_old.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%5

\captionsetup[table]{skip=6pt}

\begin{table*}[t!]
\small
\renewcommand{\arraystretch}{1.0}
\centering
{
\small
\setlength{\tabcolsep}{0.5em}
\begin{tabular}{l|l|c|cccc|ccc}
\toprule
\multirow{2}[2]{*}{\textbf{Evaluation}} & 
\multirow{2}[2]{*}{{Dataset}} & 
\multirow{2}[2]{*}{\rotatebox{90}{\emph{\notsotiny{Fine-tune}}}} & 
\multicolumn{4}{c|}{\textit{Lower is better}} &
\multicolumn{3}{c}{\textit{Higher is better}} 
\\
\cmidrule(lr){4-7} \cmidrule(lr){8-10}
& & &  
AbsRel &
SqRel &
RMSE &
RMSE$_{log}$ &
\scriptsize{$\delta < {1.25}$} &
\scriptsize{$\delta < {1.25}^2$} &
\scriptsize{$\delta < {1.25}^3$}\textbf{}
\\
\midrule
% \\
& BTS~\cite{lee2019big} & \cmark
& 0.059 & 0.245 & 2.756 & 0.096 & 0.956 & \sbestmet{\underline{0.993}} & \sbestmet{\underline{0.998}}
\\
& AdaBins~\cite{adabins} & \cmark
& 0.058 & \sbestmet{\underline{0.190}} & 2.360 & \sbestmet{\underline{0.088}} & 0.964 & \bestmet{\textbf{0.995}} & \bestmet{\textbf{0.999}}
\\
& ZoeDepth~\cite{zoedepth} & \cmark
& \sbestmet{\underline{0.057}} & 0.194 & \sbestmet{\underline{2.290}} & 0.091 & \sbestmet{\underline{0.967}} & \bestmet{\textbf{0.995}} & \bestmet{\textbf{0.999}}
\\
\cmidrule{2-10}
& & \xmark
& \bestmed{0.079} & \bestmed{0.326} & \bestmed{2.896} & \bestmed{0.120} & \bestmed{0.928} & \bestmed{0.984} & \bestmed{0.995}
\\
\multirow{-5}{*}{KITTI} & 
\multirow{-2}{*}{\textbf{\Acronym (outdoor)}} & \cmark
& \bestmet{\textbf{0.053}} & \bestmet{\textbf{0.164}} & \bestmet{\textbf{2.087}} & \bestmet{\textbf{0.083}} & \bestmet{\textbf{0.968}} & \bestmet{\textbf{0.995}} & \bestmet{\textbf{0.999}}
\\
\midrule
\midrule
& BTS~\cite{lee2019big} & \cmark
& 0.094 & 1.913 & 11.437 & 0.212 & 0.888 & 0.947 & 0.978
\\
& PackNet~\cite{packnet-san} & \cmark
& \sbestmet{\underline{0.088}} & \sbestmet{\underline{1.760}} & \sbestmet{\underline{11.331}} & \sbestmet{\underline{0.195}} & \sbestmet{\underline{0.899}} & \sbestmet{\underline{0.960}} & \sbestmet{\underline{0.981}}
\\
& ZoeDepth$^*$~\cite{zoedepth} & \xmark
& \sbestmed{0.170} & \sbestmed{3.936} & \sbestmed{19.412} & \sbestmed{0.304} & \sbestmed{0.744} & \sbestmed{0.887} & \sbestmed{0.943}
\\
\cmidrule{2-10}
& & \xmark
& \bestmed{0.102} & \bestmed{2.150} & \bestmed{11.524} & \bestmed{0.191} & \bestmed{0.829} & \bestmed{0.932} & \bestmed{0.962}
\\
\multirow{-5}{*}{DDAD (front)} & 
\multirow{-2}{*}{\textbf{\Acronym (outdoor)}} & \cmark
& \bestmet{\textbf{0.086}} & \bestmet{\textbf{1.709}} & \bestmet{\textbf{10.652}} & \bestmet{\textbf{0.180}} & \bestmet{\textbf{0.909}} & \bestmet{\textbf{0.967}} & \bestmet{\textbf{0.984}}
\\
\midrule
\midrule
& BTS~\cite{lee2019big} & \cmark
& 0.153 & 2.413 & 10.437 & 0.272 & 0.813 & \sbestmet{\underline{0.915}} & \sbestmet{\underline{0.956}}
\\
& PackNet~\cite{packnet-san} & \cmark
& \sbestmet{\underline{0.145}} & \sbestmet{\underline{2.318}} & \sbestmet{\underline{10.049}} & \sbestmet{\underline{0.242}} & \sbestmet{\underline{0.845}} & 0.909 & 0.951
\\
& ZoeDepth~\cite{zoedepth} & \xmark
& \sbestmed{0.647} & \sbestmed{8.158} & \sbestmed{16.320} & \sbestmed{0.054} & \sbestmed{0.265} & \sbestmed{0.451} & \sbestmed{0.711}  
\\
\cmidrule{2-10}
& & \xmark
& \bestmed{0.161} & \bestmed{2.633} & \bestmed{11.034} & \bestmed{0.272} & \bestmed{0.813} & \bestmed{0.912} & \bestmed{0.954}
\\
\multirow{-5}{*}{DDAD (all)} & 
\multirow{-2}{*}{\textbf{\Acronym (outdoor)}} & \cmark
& \bestmet{\textbf{0.142}} & \bestmet{\textbf{2.234}} & \bestmet{\textbf{9.842}} & \bestmet{\textbf{0.235}} & \bestmet{\textbf{0.851}} & \bestmet{\textbf{0.939}} & \bestmet{\textbf{0.967}}
\\
\midrule
\midrule
& ZoeDepth~\cite{zoedepth} & \xmark
& \sbestmed{0.504} & \sbestmed{5.015} & \sbestmed{7.717} & \sbestmed{0.461} & \sbestmed{0.255} & \sbestmed{0.659} & \sbestmed{0.848} 
\\
\cmidrule{2-10}
& & \xmark
& \bestmed{\textbf{0.255}} & \bestmed{\textbf{4.730}} & \bestmed{\textbf{7.205}} & \bestmed{\textbf{0.326}} & \bestmed{\textbf{0.746}} & \bestmed{\textbf{0.885}} & \bestmed{\textbf{0.935}}
\\
\multirow{-3}{*}{nuScenes} & 
\multirow{-2}{*}{\textbf{\Acronym (outdoor)}} & \cmark
& \bestmet{\underline{0.143}} & \bestmet{\underline{1.508}} & \bestmet{\underline{4.891}} & \bestmet{\underline{0.233}} & \bestmet{\underline{0.862}} & \bestmet{\underline{0.938}} & \bestmet{\underline{0.966}}
\\
\midrule
\midrule
& AdaBins~\cite{adabins} & \cmark
& \sbestmet{0.103} & \sbestmet{---} & \sbestmet{0.364} & \sbestmet{0.044} & \sbestmet{0.903} & \sbestmet{0.984} & \sbestmet{0.997} 
\\
& LocalBins~\cite{localbins} & \cmark
& \sbestmet{0.099} & \sbestmet{---} & \sbestmet{0.357} & \sbestmet{0.042} & \sbestmet{0.907} & \sbestmet{0.987} & \sbestmet{0.998} 
\\
& NeWCRFs~\cite{newcrfs} & \cmark
& \sbestmet{0.095} & \sbestmet{---} & \sbestmet{0.334} & \sbestmet{0.041} & \sbestmet{0.922} & \sbestmet{0.992} & \sbestmet{0.998} 
\\
& ZoeDepth~\cite{zoedepth} & \cmark
& \sbestmet{\underline{0.077}} & \sbestmet{---} & \sbestmet{\underline{0.277}} & \sbestmet{\underline{0.033}} & \sbestmet{\underline{0.953}} & \sbestmet{\underline{0.995}} & \sbestmet{\underline{0.999}} 
\\
\cmidrule{2-10}
& & \xmark
& \bestmed{0.148} & \bestmed{\underline{0.110}} & \bestmed{0.520} & \bestmed{0.179} & \bestmed{0.815} & \bestmed{0.965} & \bestmed{0.992}
\\
\multirow{-7}{*}{NYUv2} & 
\multirow{-2}{*}{\textbf{\Acronym (indoor)}} & \cmark
& \bestmet{\textbf{0.074}} & \bestmet{\textbf{0.031}} & \bestmet{\textbf{0.269}} & \bestmet{\textbf{0.103}} & \bestmet{\textbf{0.954}} & \bestmet{\textbf{0.995}} & \bestmet{\textbf{1.000}}
\\
\bottomrule
\end{tabular}
}
\caption{
\textbf{In-domain depth estimation results}, obtained by fine-tuning our outdoor \Acronym variant for a single epoch on the training splits of each evaluation dataset. The ZoeDepth$^*$ result differs from the one reported by the authors because it was calculated using the standard \emph{DDAD} evaluation protocol~\cite{packnet} (i.e., distances of up to $200$m without cropping). \emph{DDAD} and \emph{nuScenes} results are the average of all $6$ cameras, unless noted otherwise. Best and second best overall numbers are \textbf{bolded} and \underline{underlined}. Best and second best zero-shot numbers are colored in \colorbox{tabbestcolor1}{shades of red}, and best and second best fine-tuned numbers are colored in \colorbox{tabbestcolor2}{shades of green}.
}
\label{tab:finetune}
\end{table*}


